Semi-Supervised Learning of Optical Flow by Flow Supervisor

A training pipeline for optical flow CNNs consists of a pretraining stage on a synthetic dataset followed by a fine tuning stage on a target dataset. However, obtaining ground truth flows from a target video requires a tremendous effort. This paper proposes a practical fine tuning method to adapt a pretrained model to a target dataset without ground truth flows, which has not been explored extensively. Specifically, we propose a flow supervisor for self-supervision, which consists of parameter separation and a student output connection. This design is aimed at stable convergence and better accuracy over conventional self-supervision methods which are unstable on the fine tuning task. Experimental results show the effectiveness of our method compared to different self-supervision methods for semi-supervised learning. In addition, we achieve meaningful improvements over state-of-the-art optical flow models on Sintel and KITTI benchmarks by exploiting additional unlabeled datasets. Code is available at https://github.com/iwbn/flow-supervisor.

==> content/06-1_qual.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h]
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_0_im1.jpg}\caption*{}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_0_im1.jpg}\caption*{}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_0_im1.jpg}\caption*{}
 \caption{Image 1}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_0_im1.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_0_im1.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_0_im1.jpg}\caption*{}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_0_im1.jpg}\caption*{}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_0_im1.jpg}\caption*{}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_0_im1.jpg}\caption*{}
% \caption{Image 1}
% \end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_2_a_4.3672.jpg}\caption*{4.37}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_2_a_33.4225.jpg}\caption*{33.42}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_2_a_68.3838.jpg}\caption*{68.38}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_2_a_6.9717.jpg}\caption*{6.97}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_2_a_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_2_a_0.0000.jpg}\caption*{}
 \caption{RAFT}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_2_a_45.8131.jpg}\caption*{45.81}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_2_a_20.2749.jpg}\caption*{20.27}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_2_a_79.6975.jpg}\caption*{70.70}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_2_a_6.7310.jpg}\caption*{6.73}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_2_a_27.1285.jpg}\caption*{27.13}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_2_a_22.6015.jpg}\caption*{22.60}
% \caption{RAFT}
% \end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_2_b_4.3176.jpg}\caption*{4.32}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_2_b_14.4763.jpg}\caption*{14.48}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_2_b_60.6323.jpg}\caption*{60.63}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_2_b_6.8486.jpg}\caption*{6.85}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_2_b_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_2_b_0.0000.jpg}\caption*{}
 \caption{Ours}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_2_b_34.9386.jpg}\caption*{34.94}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_2_b_17.3651.jpg}\caption*{17.37}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_2_b_85.5816.jpg}\caption*{85.58}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_2_b_6.3821.jpg}\caption*{6.38}
% \end{subfigure}
% %\begin{subfigure}[b]{\linewidth}
% % \centering
% % \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_2_b_27.7249.jpg}\caption*{27.72}
% %\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_2_b_22.3339.jpg}\caption*{22.33}
% \caption{Ours}
% \end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_2_c_2.5713.jpg}\caption*{2.57}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_2_c_10.0648.jpg}\caption*{10.06}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_2_c_59.2377.jpg}\caption*{59.24}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_2_c_6.3611.jpg}\caption*{6.36}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_2_c_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_2_c_0.0000.jpg}\caption*{}
 \caption{RAFT-ft}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_2_c_17.1385.jpg}\caption*{17.14}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_2_c_8.6156.jpg}\caption*{8.62}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_2_c_49.3556.jpg}\caption*{49.36}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_2_c_5.2959.jpg}\caption*{5.30}
% \end{subfigure}
% %\begin{subfigure}[b]{\linewidth}
% % \centering
% % \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_2_c_15.2631.jpg}\caption*{15.26}
% %\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_2_c_4.6091.jpg}\caption*{4.61}
% \caption{RAFT-ft}
% \end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_2_d_2.0861.jpg}\caption*{2.09}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_2_d_7.4480.jpg}\caption*{7.45}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_2_d_56.6237.jpg}\caption*{56.62}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_2_d_4.2682.jpg}\caption*{4.27}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_2_d_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_2_d_0.0000.jpg}\caption*{}
 \caption{Ours-ext}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_2_d_15.2206.jpg}\caption*{15.22}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_2_d_7.1779.jpg}\caption*{7.18}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_2_d_48.2222.jpg}\caption*{48.22}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_2_d_4.1987.jpg}\caption*{4.20}
% \end{subfigure}
% %\begin{subfigure}[b]{\linewidth}
% % \centering
% % \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_2_d_14.3482.jpg}\caption*{14.35}
% %\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_2_d_3.8206.jpg}\caption*{3.82}
% \caption{Ours-ext}
% \end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/16_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/1_1_gt.jpg}\caption*{}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/2_1_gt.jpg}\caption*{}
%\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_compare/3_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/171_1_gt.png}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/sintel_t_compare/357_1_gt.png}\caption*{}
 \caption{Ground-truth}
\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/4_1_gt.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/5_1_gt.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/sintel_compare/6_1_gt.jpg}\caption*{}
%\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/7_1_gt.jpg}\caption*{}
% \end{subfigure}
% %\begin{subfigure}[b]{\linewidth}
% % \centering
% % \includegraphics[width=\linewidth]{figure/qual/sintel_compare/8_1_gt.jpg}\caption*{}
% %\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/sintel_compare/9_1_gt.jpg}\caption*{}
% \caption{Ground-truth}
% \end{subfigure}
\end{minipage}
\centering
\caption{\textbf{Results on Sintel Final.} In this table, RAFT (b) and RAFT-ft (d) are tested from pretrained models by RAFT authors, where RAFT-ft uses Sintel for fine-tuning. Ours (c) uses FlyingThings3D as a labeled dataset and Sintel as an unlabeled dataset.
For Ours-ext (e), we use Sintel as labeled and Spring as unlabeled, as in Table~5 in the main paper. 
The top 3 rows are from the training set of Sintel final, where we show EPEs under predictions. The last two rows show the test results with ground-truth, which can be obtained from Sintel benchmark site~\cite{SintelBenchmarkSite}. 
Note that the magnitude normalization (saturation) is different in the test-set ground-truth visualizations because real optical flow values are not accessible.
On Sintel, improvements are observed in RAFT (b) $\rightarrow$ Ours (c). We can observe L2L-Flow successfully recover the left hand of the man (4-th row), and the right wing of the dragon (5-th row).
Interestingly, fine-tuning with the supervised dataset, i.e., RAFT-ft,
(d) sometimes degrades the performance on test samples; the end of the sphere (4-th row), and the sky region (5-th row).
By using additional videos without a label, i.e., Ours-ext (e), we observe it can prevent the degradation and take advantage of the labeled data by showing clear boundary too.  
}
\label{fig:sintel}
\end{figure*}
\vfill

\begin{figure*}[h]
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_0_im1.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_0_im1.jpg}\caption*{}
 \caption{Image 1}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_0_im1.jpg}\caption*{}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_0_im1.jpg}\caption*{}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_0_im1.jpg}\caption*{}
% \caption{Image1}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_0_im1.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_0_im1.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_0_im1.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_0_im1.jpg}\caption*{}
%\caption{Image 1}
%\end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_2_a_5.4919.jpg}\caption*{5.49}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_2_a_2.0480.jpg}\caption*{2.05}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_2_a_4.2397.jpg}\caption*{4.24}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_2_a_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_2_a_0.0000.jpg}\caption*{}
 \caption{RAFT}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_2_a_2.6028.jpg}\caption*{2.60}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_2_a_2.2703.jpg}\caption*{2.27}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_2_a_6.0001.jpg}\caption*{6.00}
% \caption{RAFT}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_2_a_2.6837.jpg}\caption*{2.68}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_2_a_9.4762.jpg}\caption*{9.48}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_2_a_1.7782.jpg}\caption*{1.78}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_2_a_5.7641.jpg}\caption*{5.76}
%\end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_2_b_5.5325.jpg}\caption*{5.53}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_2_b_1.1018.jpg}\caption*{1.10}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_2_b_3.6487.jpg}\caption*{3.65}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_2_b_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_2_b_0.0000.jpg}\caption*{}
 \caption{Ours}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_2_b_2.1319.jpg}\caption*{2.13}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_2_b_1.9947.jpg}\caption*{1.99}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_2_b_4.8503.jpg}\caption*{4.85}
% \caption{Ours}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_2_b_2.4169.jpg}\caption*{2.42}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_2_b_8.6787.jpg}\caption*{8.68}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_2_b_1.7669.jpg}\caption*{1.77}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_2_b_5.4218.jpg}\caption*{5.42}
%\end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_2_c_7.0121.jpg}\caption*{7.01}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_2_c_3.5461.jpg}\caption*{3.55}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_2_c_2.4710.jpg}\caption*{2.47}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_2_c_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_2_c_0.0000.jpg}\caption*{}
 \caption{RAFT-ft}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_2_c_2.0625.jpg}\caption*{2.06}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_2_c_1.6917.jpg}\caption*{1.69}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_2_c_1.8712.jpg}\caption*{1.87}
% \caption{RAFT-ft}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_2_c_2.0820.jpg}\caption*{2.08}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_2_c_4.4898.jpg}\caption*{4.49}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_2_c_1.2343.jpg}\caption*{1.23}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_2_c_3.0396.jpg}\caption*{3.04}
%\end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_2_d_2.1531.jpg}\caption*{2.15}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_2_d_1.6685.jpg}\caption*{1.67}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_2_d_1.8156.jpg}\caption*{1.82}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_2_d_0.0000.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_2_d_0.0000.jpg}\caption*{}
 \caption{Ours-ext}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_2_d_1.4952.jpg}\caption*{1.50}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_2_d_1.2525.jpg}\caption*{1.25}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_2_d_1.4693.jpg}\caption*{1.47}
% \caption{Ours-ext}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_2_d_1.7169.jpg}\caption*{1.72}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_2_d_4.1647.jpg}\caption*{4.16}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_2_d_0.9636.jpg}\caption*{0.96}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_2_d_2.7805.jpg}\caption*{2.78}
%\end{subfigure}
\end{minipage}
\begin{minipage}{.16\textwidth}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/0_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/1_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/2_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/42_1_gt.jpg}\caption*{}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
 \centering
 \includegraphics[width=\linewidth]{figure/qual/kitti_t_compare/174_1_gt.jpg}\caption*{}
 \caption{Ground-truth}
\end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/3_1_gt.jpg}\caption*{}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/4_1_gt.jpg}\caption*{}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/5_1_gt.jpg}\caption*{}
% \caption{Ground-truth}
% \end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/6_1_gt.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/7_1_gt.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/8_1_gt.jpg}\caption*{}
%\end{subfigure}
%\begin{subfigure}[b]{\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/qual/kitti12_compare/9_1_gt.jpg}\caption*{}
%\caption{Ground-truth}
%\end{subfigure}
\end{minipage}
\centering
\caption{\textbf{Results on KITTI.} In this table, RAFT (b) and RAFT-ft (d) are tested from pretrained models by RAFT authors, where RAFT-ft uses KITTI 2015 for fine-tuning. Ours (c) uses FlyingThings3D as a labeled dataset and KITTI-multiview as an unlabeled dataset.
For Ours-ext (e), we use KITTI 2015 as labeled and KITTI-multiview as unlabeled, as in Table~5 in the main paper. The top 3 rows are from the training set of KITTI 2012, where we show EPEs under predictions. The last two rows show the test results without ground-truth.
Results on KITTI show not distinctive representation in qualitative results; the ground-truth flows are sparse, and scenes are pretty simple usually.
Still, we can observe meaningful improvement in EPEs when our method is used.
In the 4-th row, we bring an example with a person on a bike.
Specifically for the bike, the optical flow boundary is much accurate when ground-truth is not used (b-c),
while (d) degrades the boundary of the bike.
Ours-ext (c), which is a semi-supervised approach,
partly relieves the boundary issues.
}
\label{fig:kitti}
\end{figure*}
\pagebreak

==> content/figure_tex/qual_kitti.tex <==
%\begin{figure}[t]
\begin{wrapfigure}[14]{r}{0.5\textwidth}
\centering
\begin{subfigure}[b]{0.322\linewidth}
    \centering
    \includegraphics[trim={0mm 165.9mm 213.25mm 0mm},clip,width=\linewidth]{figure/qual_combined.pdf}
    \caption{Input}
\end{subfigure}
\begin{subfigure}[b]{0.322\linewidth}
    \centering
    \includegraphics[trim={40.75mm 165.9mm 172.5mm 0mm},clip,width=\linewidth]{figure/qual_combined.pdf}
    \caption{Sup.}
\end{subfigure}
\begin{subfigure}[b]{0.322\linewidth}
    \includegraphics[trim={81.5mm 165.9mm 131.75mm 0mm},clip,width=\linewidth]{figure/qual_combined.pdf}
    \caption{Ours}
\end{subfigure}

\caption{\textbf{Qualitative results on KITTI testing samples.} We compare the supervised model (Sup) with the semi-supervised model (Ours). Both models 
exploit KITTI labels; ours utilizes additional unlabeled KITTI for fine tuning}
\label{fig:qual_kitti}
%\end{figure}
\end{wrapfigure}

